FDTD-Based Diffuse Scattering and Transmission Models for Ray-Tracing of Millimeter-Wave Communication Systems

At millimeter-wave frequencies, diffuse scattering from rough surfaces is an important propagation mechanism. Including this mechanism in radio propagation modeling tools,such as ray-tracing, is a key step towards realizing accurate propagation models for 5G and beyond systems. We propose a two-stage solution to this problem. First, we model reflection and transmission through rough slabs, such as doors, walls and windows with the FDTD method. Our results indicate the influence of roughness and whether this influence is measurable, either reducing the magnitude of the reflected and transmitted waves, or (most importantly) generating diffuse scattering components. In the latter case, the surface effectively acts as a secondary source, whose pattern is computed by full-wave analysis. Then, this pattern is embedded in a ray-tracer, enabling the computation and tracing of diffuse scattering field components. We demonstrate this approach in the ray-tracing analysis of a 28 GHz indoor environment.

==> Proxeiro.tex <==
\begin{equation}
\frac{\partial E^y}{\partial z} = -\mu_0\frac{\partial H^x}{\partial t}
 \label{eq:Aux1}
\end{equation}


 \begin{equation}
\frac{\partial H^x}{\partial z} =-\sigma E^y -\epsilon_0(\epsilon_r' - sin^2\theta_i)\frac{\partial Ε^y}{\partial t}
 \label{eq:Aux2}
\end{equation}

 \begin{equation}
    H^z= \frac{sin\theta_i H^z }{Z_o}
     \label{eq:Aux3}
\end{equation}


\begin{figure*}[!htb]\centering
\centering
 



\begin{figure}[h]
 \begin{tikzpicture}
\centering
  \node at(0,0)  {\includegraphics[scale=0.42]{Heights.pdf}};


%\node at (-2.4,0.8) [align=left] {\scalebox{0.5}{Upper Layer}};
%\node at (-2.4,0) [align=left] {\scalebox{0.5}{Medium Layer}};
%\node at (-2.4,-0.5) [align=left] {\scalebox{0.5}{Lower Layer}};

\end{tikzpicture}
\caption{{Critical heights for a plane wave propagating from a dielectric to air}}
 \label{fig:Heights}
\end{figure}








begin{figure*}[!t]
\centering
 \begin{tikzpicture}
\node at (-10.5,0) [align=left] {\scalebox{1}{Reflection pattern}};
\node at (-6.5,0) [align=left] {\scalebox{1}{Transmission pattern}};
\node at (-2,0) [align=left] {\scalebox{1}{Reflection pattern}};
\node at (1.5,0) [align=left] {\scalebox{1}{Transmission pattern}};

\end{tikzpicture}

    \subfigure[Case at which specular is attenuated, $\sigma_h =$ 1 mm]
    {\label{fig:R_T_1}
    \includegraphics[scale=0.6]{Cnc_R_T_1.pdf}}
    \subfigure[Case at which specular is vanished, $\sigma_h =$ 6 mm]
    {\label{fig:R_T_2}
    \includegraphics[scale=0.6]{Cnc_R_T_2.pdf}}
\caption{{Reflection (a) from and transmission (b) patterns through a 20 cm rough concrete slab at 28 GHz}}

\end{figure*}

    {\includegraphics[scale=1]{Cnc_all.pdf}}
    \caption{{Reflection (a) from and transmission (b) patterns through a 20 cm rough concrete slab at 28 GHz}}
    \label{fig:Cnc_all}


For the left and right boundary, this is equivalent to introducing a constant time delay  $ \Delta\tau= cx_{\text{\tiny TFSF}}_{\text{\tiny 1,2}} /\sin\theta_i$ respectively, to the stored values of the nodes that are found between $z_{\text{\tiny TFSF}}_{\text{\tiny 1}}$ and  $z_{\text{\tiny TFSF}}_{\text{\tiny 2}}$.  For the bottom and top boundary this is equivalent to introducing a 


For the left and right boundary, this is equivalent to introducing a constant time delay  $ \Delta\tau= cx_{\text{\tiny TFSF}}_{\text{\tiny 1,2}} /\sin\theta_i$ respectively, to the stored values of the nodes that are found between $z_{\text{\tiny TFSF}}_{\text{\tiny 1}}$ and  $z_{\text{\tiny TFSF}}_{\text{\tiny 2}} - 1$ .  For the bottom and top boundary this is equivalent to introducing a  $ \Delta\tau= cx_i /\sin\theta_i$, where $x_i$ is between $x_{\text{\tiny TFSF}}_{\text{\tiny 1}}$ and $x_{\text{\tiny TFSF}}_{\text{\tiny 2}}$ , to the stored values of the nodes that are found at and  $z_{\text{\tiny TFSF}}_{\text{\tiny 2}} $ and $z_{\text{\tiny TFSF}}_{\text{\tiny 2}} $ respectively 
